Memory Triggers: Unveiling Memorization in Text-To-Image Generative Models through Word-Level Duplication

Diffusion-based models, such as the Stable Diffusion model, have revolutionized text-to-image synthesis with their ability to produce high-quality, high-resolution images. These advancements have prompted significant progress in image generation and editing tasks. However, these models also raise concerns due to their tendency to memorize and potentially replicate exact training samples, posing privacy risks and enabling adversarial attacks. Duplication in training datasets is recognized as a major factor contributing to memorization, and various forms of memorization have been studied so far. This paper focuses on two distinct and underexplored types of duplication that lead to replication during inference in diffusion-based models, particularly in the Stable Diffusion model. We delve into these lesser-studied duplication phenomena and their implications through two case studies, aiming to contribute to the safer and more responsible use of generative models in various applications.

==> sec/copied_fig_ast.tex <==
\begin{figure*}[h]
    \centering
    \begin{adjustbox}{width=16cm,center}
    \begin{tabular}{m{4cm}>{\centering\arraybackslash}m{2cm}*{4}{m{2cm}}>{\centering\arraybackslash}m{2cm}}
        \hline
        \centering \textbf{Prompt} & \centering \textbf{Text Similarity} & \multicolumn{4}{c}{\textbf{Example Generated Images}} & \textbf{US Flag \%} \\
        \hline
        \raggedright A child \textcolor{red}{astronaut} riding a dog through space  & 0.7669 & 
        \includegraphics[width=2cm,height=2cm]{AuthorKit24/AnonymousSubmission/LaTeX/sec/astronaut/5.pdf} &
        \includegraphics[width=2cm,height=2cm]{AuthorKit24/AnonymousSubmission/LaTeX/sec/astronaut/6.pdf} &
        \includegraphics[width=2cm,height=2cm]{AuthorKit24/AnonymousSubmission/LaTeX/sec/astronaut/7.pdf} &
        \includegraphics[width=2cm,height=2cm]{AuthorKit24/AnonymousSubmission/LaTeX/sec/astronaut/8.pdf} &
        24\% \\
        \hline
        \raggedright A group of \textcolor{red}{astronauts} in training inside a mock spacecraft. & 0.6227 & 
        \includegraphics[width=2cm,height=2cm]{AuthorKit24/AnonymousSubmission/LaTeX/sec/astronaut/2.pdf} &
        \includegraphics[width=2cm,height=2cm]{AuthorKit24/AnonymousSubmission/LaTeX/sec/astronaut/3.pdf} &
        \includegraphics[width=2cm,height=2cm]{AuthorKit24/AnonymousSubmission/LaTeX/sec/astronaut/5(1).pdf} &
        \includegraphics[width=2cm,height=2cm]{AuthorKit24/AnonymousSubmission/LaTeX/sec/astronaut/7(1).pdf} &
        47\% \\
        \hline
        \raggedright A Chinese \textcolor{red}{astronaut} performing a spacewalk from the shuttle to test new satellite repair technologies. & 0.6093 & 
        \includegraphics[width=2cm,height=2cm]{AuthorKit24/AnonymousSubmission/LaTeX/sec/astronaut/5(2).pdf} &
        \includegraphics[width=2cm,height=2cm]{AuthorKit24/AnonymousSubmission/LaTeX/sec/astronaut/3(1).pdf} &
        \includegraphics[width=2cm,height=2cm]{AuthorKit24/AnonymousSubmission/LaTeX/sec/astronaut/6(1).pdf} &
        \includegraphics[width=2cm,height=2cm]{AuthorKit24/AnonymousSubmission/LaTeX/sec/astronaut/8(1).pdf} &
        63.4\% \\
        \hline
        \raggedright An \textcolor{red}{astronaut} wearing a Russian Orlan spacesuit during a spacewalk. & 0.7390 & 
        \includegraphics[width=2cm,height=2cm]{AuthorKit24/AnonymousSubmission/LaTeX/sec/astronaut/2(1).pdf} &
        \includegraphics[width=2cm,height=2cm]{AuthorKit24/AnonymousSubmission/LaTeX/sec/astronaut/3(2).pdf} &
        \includegraphics[width=2cm,height=2cm]{AuthorKit24/AnonymousSubmission/LaTeX/sec/astronaut/4.pdf} &
        \includegraphics[width=2cm,height=2cm]{AuthorKit24/AnonymousSubmission/LaTeX/sec/astronaut/5(3).pdf} &
        97.8\% \\
        \hline
    \end{tabular}
    \end{adjustbox}
    \caption{Prompts and their corresponding generated images with the percentage of images containing the US flag.}
    \label{fig:us_flag_examples}
\end{figure*}

==> sec/fig5.tex <==




\begin{figure*}[h]
    \centering
    \begin{adjustbox}{width=\textwidth,center}
    \begin{tabular}{|m{4cm}|>{\centering\arraybackslash}m{1.5cm}|>{\centering\arraybackslash}m{2cm}|*{3}{m{2cm}|}m{2cm}|}
        \hline
        \multirow{2}{*}{\centering \textbf{Prompt}} & \multirow{2}{*}{\parbox{1.5cm}{\centering \textbf{Text\\Similarity}}} & \multirow{2}{*}{\parbox{2cm}{\centering \textbf{Image Sim $>$ 0.82 (\%)}}} & \multicolumn{3}{c|}{\textbf{Example Generated Images}} & \multirow{2}{*}{\parbox{2cm}{\centering \textbf{Original Image}}} \\
        \cline{4-7}
        & & & \textbf{$>$ 0.82} & \textbf{0.75-0.82}  & \textbf{$<$0.75} & \\
        \hline
        \raggedright Van Gogh cafe terrace & 1.0000 & 90.4\% & 
        \raisebox{-0.05\height}{\includegraphics[width=2cm]{AuthorKit24/AnonymousSubmission/LaTeX/sec/cafe_terrace/selected_image_7.pdf}} &
        \raisebox{-0.05\height}{\includegraphics[width=2cm]{AuthorKit24/AnonymousSubmission/LaTeX/sec/cafe_terrace/selected_image_109.pdf}} &
        \raisebox{-0.05\height}{\includegraphics[width=2cm]{AuthorKit24/AnonymousSubmission/LaTeX/sec/cafe_terrace/selected_image_327.pdf}} &
        \raisebox{-0.05\height}{\includegraphics[width=2cm]{AuthorKit24/AnonymousSubmission/LaTeX/sec/cafe_terrace/cafe_terrace.pdf}}\\
        \hline
        \raggedright A serene \textcolor{red}{cafe terrace} blending into a \textcolor{red}{van Gogh} landscape. & 0.8279 & 39\% &
        \raisebox{-0.05\height}{\includegraphics[width=2cm]{AuthorKit24/AnonymousSubmission/LaTeX/sec/cafe_terrace/selected_image_482.pdf}} &
        \raisebox{-0.05\height}{\includegraphics[width=2cm]{AuthorKit24/AnonymousSubmission/LaTeX/sec/cafe_terrace/selected_image_62.pdf}} &
        \raisebox{-0.05\height}{\includegraphics[width=2cm]{AuthorKit24/AnonymousSubmission/LaTeX/sec/cafe_terrace/selected_image_473.pdf}} &
        \raisebox{-0.05\height}{\includegraphics[width=2cm]{AuthorKit24/AnonymousSubmission/LaTeX/sec/cafe_terrace/cafe_terrace.pdf}}\\
        \hline
        \raggedright Sunlight filters through the leaves onto a \textcolor{red}{cafe terrace}, casting playful shadows over the scene as if inviting \textcolor{red}{van Gogh} to capture its simple beauty. & 0.7323 & 22.2\% &
        \raisebox{-0.05\height}{\includegraphics[width=2cm]{AuthorKit24/AnonymousSubmission/LaTeX/sec/sunflowers/selected_image_212.pdf}} &
        \raisebox{-0.05\height}{\includegraphics[width=2cm]{AuthorKit24/AnonymousSubmission/LaTeX/sec/sunflowers/selected_image_225.pdf}} &
        \raisebox{-0.05\height}{\includegraphics[width=2cm]{AuthorKit24/AnonymousSubmission/LaTeX/sec/sunflowers/selected_image_360.pdf}} &
        \raisebox{-0.05\height}{\includegraphics[width=2cm]{AuthorKit24/AnonymousSubmission/LaTeX/sec/sunflowers/sunflowers.pdf}}\\
        \hline
        \raggedright The new video game features a level where you collect \textcolor{red}{sunflowers} to unlock a character called \textcolor{red}{Van Gogh}. & 0.5690 & 25.8\% &
        \raisebox{-0.05\height}{\includegraphics[width=2cm]{AuthorKit24/AnonymousSubmission/LaTeX/sec/sunflowers/selected_image_216.pdf}} &
        \raisebox{-0.05\height}{\includegraphics[width=2cm]{AuthorKit24/AnonymousSubmission/LaTeX/sec/sunflowers/selected_image_203.pdf}} &
        \raisebox{-0.05\height}{\includegraphics[width=2cm]{AuthorKit24/AnonymousSubmission/LaTeX/sec/sunflowers/selected_image_378.pdf}} &
        \raisebox{-0.05\height}{\includegraphics[width=2cm]{AuthorKit24/AnonymousSubmission/LaTeX/sec/sunflowers/sunflowers.pdf}}\\
        \hline
        % Add more rows as needed
    \end{tabular}
    \end{adjustbox}
    \caption{Captions and their corresponding generated images for different seeds.}
    \label{fig:terrace}
\end{figure*}

==> sec/fig7.tex <==
\begin{figure*}[h]
    \centering
    \begin{tabular}{|m{4cm}|*{4}{m{2cm}|}m{2cm}|}
        \hline
        \textbf{Prompt} & \multicolumn{4}{c|}{\textbf{Generated Images}} & \textbf{Percentage of Images Containing the US Flag} \\
        \hline
        \raggedright Prompt 1 & 
        \includegraphics[width=2cm]{path/to/image1.pdf} &
        \includegraphics[width=2cm]{path/to/image2.pdf} &
        \includegraphics[width=2cm]{path/to/image3.pdf} &
        \includegraphics[width=2cm]{path/to/image4.pdf} &
        XX\% \\
        \hline
        \raggedright Prompt 2 & 
        \includegraphics[width=2cm]{path/to/image5.pdf} &
        \includegraphics[width=2cm]{path/to/image6.pdf} &
        \includegraphics[width=2cm]{path/to/image7.pdf} &
        \includegraphics[width=2cm]{path/to/image8.pdf} &
        XX\% \\
        \hline
        \raggedright Prompt 3 & 
        \includegraphics[width=2cm]{path/to/image9.pdf} &
        \includegraphics[width=2cm]{path/to/image10.pdf} &
        \includegraphics[width=2cm]{path/to/image11.pdf} &
        \includegraphics[width=2cm]{path/to/image12.pdf} &
        XX\% \\
        \hline
        \raggedright Prompt 4 & 
        \includegraphics[width=2cm]{path/to/image13.pdf} &
        \includegraphics[width=2cm]{path/to/image14.pdf} &
        \includegraphics[width=2cm]{path/to/image15.pdf} &
        \includegraphics[width=2cm]{path/to/image16.pdf} &
        XX\% \\
        \hline
        \raggedright Prompt 5 & 
        \includegraphics[width=2cm]{path/to/image17.pdf} &
        \includegraphics[width=2cm]{path/to/image18.pdf} &
        \includegraphics[width=2cm]{path/to/image19.pdf} &
        \includegraphics[width=2cm]{path/to/image20.pdf} &
        XX\% \\
        \hline
    \end{tabular}
    \caption{Comparison of various prompts and the percentage of generated images containing the US flag.}
    \label{fig:us_flag_study}
\end{figure*}

